Learning general and distinctive 3D local deep descriptors for point cloud registration

An effective 3D descriptor should be invariant to different geometric transformations, such as scale and rotation, robust to occlusions and clutter, and capable of generalising to different application domains. We present a simple yet effective method to learn general and distinctive 3D local descriptors that can be used to register point clouds that are captured in different domains. Point cloud patches are extracted, canonicalised with respect to their local reference frame, and encoded into scale and rotation-invariant compact descriptors by a deep neural network that is invariant to permutations of the input points. This design is what enables our descriptors to generalise across domains. We evaluate and compare our descriptors with alternative handcrafted and deep learning-based descriptors on several indoor and outdoor datasets that are reconstructed by using both RGBD sensors and laser scanners. Our descriptors outperform most recent descriptors by a large margin in terms of generalisation, and also become the state of the art in benchmarks where training and testing are performed in the same domain.

==> sections/bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{resources/bio_photos/fabio}}]{Fabio Poiesi}
is a Research Scientist in the Technologies of Vision (TeV) Lab at Fondazione Bruno Kessler in Trento, Italy.
He received his Ph.D.~degree in Electronic Engineering and Computer Science from Queen Mary University of London (UK) in March 2014. 
He spent nearly three years as a Postdoctoral Researcher in Queen Mary University of London before moving to TeV.
His research interests are 3D scene understanding, object detection and tracking, localisation and mapping, and extended reality.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{resources/bio_photos/davide}}]{Davide Boscaini}
is a Research Scientist in the Technologies of Vision (TeV) Lab at Fondazione Bruno Kessler in Trento, Italy. 
He received his Ph.D.~degree in Computational Science from Università della Svizzera Italiana (USI) in Lugano (CH) in August 2017. 
His main research interests are 3D computer vision and 3D deep learning. 
He is credited as one of the pioneers of geometric deep learning, an extension of deep learning techniques to unstructured data such as 3D point clouds and graphs.
% , an author of several papers and inventor of three US patents on the topic.
% He is the inventor of two US patents on these topics that were later acquired by Twitter Inc. in 2020.
\end{IEEEbiography}

